Teaching Program Decomposition in CS1: A Conceptual Framework for Improved Code Quality

Program decomposition is essential for developing maintainable and efficient software, yet it remains a challenging skill to teach and learn in introductory programming courses. What does program decomposition for procedural CS1 programs entail? How can CS1 students improve the decomposition of their programs? What scaffolded exercises can instructors use to teach program decomposition skills? We aim to answer all these questions by presenting a conceptual framework that (1) is grounded in the established code style principles, (2) provides a systematic approach that can be taught to students as an actionable strategy to improve the program decomposition of their programs, and (3) includes scaffolded exercises to be used in classroom activities. In addition, this systematic approach is automatable and can further be used to implement visualizers, automated feedback generators and digital tutors.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> paper_sections/not_used/Metric_Validation.tex <==
% 1. reason about scoring (not done), theoretically sound for now 
% 2. generalizable (perfomance is consistent)
% 3. extrapolation (apply to the worl scenario)
% 4. 

\section{Metric Validation}
\subsection{Distilled Description of Kane's Framework}
For the evaluation of our proposed automated metric of procedural decomposition, similar to Nelson et al. in their evaluation of formative CS assignments \cite{NelsonValidatingAssignment2019}, we validate our metric with Kane's framework for the creation and evaluation of Interpretation/Use arguments (IUAs) for validating test scores \cite{kaneTestEvaluation}. Under this framework, the evaluation criteria are dependent on the strength of the claims of the interpretation. Thus, more ambitious interpretations of test results require a larger body of evidence. Additionally, in the evaluation of the test, assumptions related to the scoring, generalization, and extrapolation of the evaluation model are addressed. Kane's framework additionally provides guidelines regarding decision-making based on the test results.

In this section, we present a conservative IUA for the current testing procedure and address the relevant assumptions of our interpretation. We additionally lay out an expanded IUA and outline the further work needed for the validation of the more ambitious interpretation.

\subsection{Conservative Interpretation and Assumptions}
Given our limited application of the current scoring schema to a relatively small sample (N = 37) of student submissions for the garden problem described above, we interpret the score as an indicator of the student's understanding of the specific decomposition principles previously outlined. We do not present it as a complete measure of procedural decomposition quality, nor do we recommend its application to a wider problem space without further validation. With regard to the principles of decomposition that we do address, we present an argument for the theoretical soundness of the measurements.

First, by comparing student solutions to an expert-written, optimally decomposed solution, we provide context to measurements that otherwise cannot currently be evaluated in the methods we find most appropriate for the project. For example, whether or not a program has the opportunity for reusable structures is inherently problem-specific, and thus cannot be punished or rewarded without context.

\subsubsection{Scoring}
Each of our 4 outlined measurements is closely linked to the principles of decomposition outlined in our framework. Minimizing global code volume is a clear prerequisite for appropriate function design. Functions that both print and return values constitute clear violations of the single responsibility principle. Functions that rely on large amounts of data to be aggregated represent potentially sub-optimal levels of information passing. The presence of low-abstraction functions invoked by distinct high-abstraction functions is a clear application of reusability. 
\subsubsection{Generalization}
Generalization refers to how representative a given test score is of the student's average test score of the universe of similar tests. Given the limited scope of problems applicable to a standard CS1 class, we expect limited variation in student performance across assignments, assuming a lack of further instruction and feedback. However, given that the assessments are presented as week-long homework assignments, variation in student code quality as a result of varied time commitments to the project is expected. Thus if the effort level is not held constant, the generalization of any given test instance is limited. 
\subsubsection{Extrapolation}
Regarding extrapolation to a broader, non-test, domain, although there are significant differences between CS1 assignments and standard industry projects, the decomposition skills demonstrated in a simple context suggest the ability to continue to apply them as software expands. 

\subsubsection{Summary}
Given that our interpretation only claims that our test gives an accurate representation of the student's understanding of the outlined principles, and our measurements are linked to these outlined principles, we hold this interpretation as sound and propose its use be limited to instructor feedback and research analysis, but not yet applied to the grading of student work.

\subsection{Future Work}
More assessments of the dependency framework are necessary to ensure its validity and reliability. More work is needed to generalize the dependency framework and accompanying step-by-step procedures to more complicated problems. The test data that the system has been exposed to so far has been relatively simple; none of it has had complicated control flow, manipulated complex data types, or possessed nested function definitions.

The value of the test score increases significantly if we can confidently interpret it as a holistic measure of decomposition quality. To achieve this, future work is needed in the refinement of the scoring method and exploration of the predictive qualities of the score.

\subsubsection{Refinement approaches}
Improvement to the scoring metric requires the exploration of other data points related to the outlined principles and a generalization of the scoring schema to enable testing without the presence of an optimally generated solution. This process would require an empirical examination of optimal ranges for the metrics we've outlined so that they can scale appropriately with the problem size.

Additionally, empirical verification of the efficacy of the scoring schema would improve confidence in our interpretation. Analysis comparing automated scores to expert-generated analysis, statistical analysis of the correlation between score and qualitatively demonstrated student understanding, and predictive analysis of the score with relation to larger-scale code quality evaluations, would all provide substantive evidence of the validity of the scoring method.



==> paper_sections/not_used/findings.tex <==
\section{Findings}

%RQs are typically defined in the introduction section and %answered in the findings sectioned, why are they originally
%defined here
Research questions:

\begin{itemize}
    \item What process do students follow when working on the PD problems? (themes, potentially correlating with performance on the exam)
    \item How does the performance on the exam correlate to the performance on the homework?
    \item 
\end{itemize}

\subsection{Applying the proposed procedure to the 12 multi-function assignments in CS1}

\subsection{RQ 2}
In our analysis of student solutions to the garden problem and their performance on the decomposition problem on the midterm exam, we report no correlation (r = .005, N = 37). This suggests that the skills required for successful procedural decomposition vary widely depending on the context of the problem. For homework assignments, students are provided a week to complete their submission, and have regular access to help in the form of IDEs, online resources, TAs, and office hours. During a midterm, the high amount of time pressure leads to a greater focus on technical details that are relatively trivial than is present in the more relaxed homework context. 

As a result of this distinction, our scoring metrics for the homework questions and exams related to different stages of the decomposition process. The lack of correlation between our scoring schemas potentially suggests that students develop these skill-sets largely independently, and thus pedagogical approaches to each component require further study.



==> paper_sections/not_used/methodology.tex <==
\section{Methodology}

\subsection{CS1 Sample Curriculum Case Study}
All 8 of the presented assignments were designed to highlight procedural decomposition as a key component. For several of the provided problems, this was achieved by providing students with globally scoped solutions and requiring them to decompose the code into appropriate functions. Prior to completing the assignments, students were exposed to the procedures outlined in \ref{subsec:procedure} and \ref{subsec:automated_procedure}. 

The assignments were included within the standard curriculum for the CS1 course, and simplified similar problems were included in summative exams to further enforce procedural decomposition as a foundational skill.

In table \ref{table:assignments} the assignments are labeled with associated procedural decomposition features, and in figures \ref{fig:var_dec_box}, \ref{fig:var_dec_drive}, and \ref{fig:var_dec_garden}, the application of the variable dependency graph is shown. 


\input{tables/assignment_features}

Specific components represent higher abstraction functions that are responsible for a significant portion of the program's total functionality. Reusable structures are distinguished from utility functions by the feature that reusable structures serve to abstract logic or computation used by a specific component of the program, while utility functions were accessed in multiple, separate components within the program. Data-processing stages refer to the processes required to handle programming-specific tasks that were necessary to complete the program's functionality.

\subsection{Garden Problem Case Study}
\label{subsec:garden_case_study}

As seen in table \ref{table:assignments}, the Garden Problem possesses three of the discussed decomposition features. It contains (1) a sequence of distinct operations, (2) functions that can be used multiple times with slight changes to input, and (3) functions which solve self-contained problems. As a result, the Garden Problem served as the best indicator of procedural validity. 

\begin{comment}
\begin{figure*}
\includegraphics[scale = .15]{images/reduced_graph_box.png}
\caption{Illustrating the proposed procedure for the Box Problem}
\label{fig:var_dec_box}
\end{figure*}

\begin{figure*}
\includegraphics[scale = .15]{images/reduced_graph_drive.png}
\caption{Illustrating the proposed procedure for the Drive Problem}
\label{fig:var_dec_drive}
\end{figure*}

\begin{figure*}
\includegraphics[scale = .15]{images/reduced_graph_garden.png}
\caption{Illustrating the proposed procedure for the Garden Problem}
\label{fig:var_dec_garden}
\end{figure*}
\end{comment}

\begin{center}
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/reduced_graph_box.png}
        \captionof{figure}{proposed procedure for the Box problem}
        \label{fig:var_dec_box}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/reduced_graph_drive.png}
        \captionof{figure}{proposed procedure for the Drive Times problem}
        \label{fig:var_dec_drive}
    \end{minipage}
    \par 
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/reduced_graph_garden.png}
        \captionof{figure}{proposed procedure for the Garden problem}
        \label{fig:var_dec_garden}
    \end{minipage}
    \hfill
\end{center}

\subsection{Justifications for Decomposition Features}

The logic behind the separation of code segments in terms of information dependency comes from both the desire to reduce artificial coupling and from past research into program slicing. In Ardalani et al., for example, the researchers divided lines of code into methods based upon the output statements that they affected \cite{ardalani2023supporting}. Similarly to identifying reusable structures and utility functions in this paper's dependency graphs, this technique improves the overall structure of the program by making the functions both more understandable (and therefore less complex) and more cohesive.

The need to isolate components implemented multiple times for different nodes into functions with parameters that represent the differing inputs is reflected by the single responsibility principle and by the desire to maximize reuse. If the shared node can be easily defined as a process with one purpose that is separate from the components that use it, then it should be abstracted away from them in order to maintain functional cohesion. If this shared component is then implemented multiple times, then it demonstrates a design with reuse kept in mind. If the shared function is organized well, this will increase the program's overall reusability.

\subsection{Principles for Assignment Generation}



==> tables/assignment_features.tex <==
\begin{table}[h]
\begin{tabular}{|>{\raggedright}p{3cm}|>{\raggedright\arraybackslash}p{3cm}|}
  \hline
  \textbf{Problem} & \textbf{Decomposition Feature} \\ \hline
  Guitar  &  \\ \hline
  Old MacDonald & \\ \hline
  Flower Buds and Steams & \\ \hline
  One little elephant  &  \\ \hline
  Fish  &  \\ \hline
  Tower  & Discrete Components \\ \hline
  Owls  & Utility Function \\ \hline
  Rubik's Cube & Reusable Structure \\ \hline
  Basic Statistics  &  Discrete Components \\ \hline
  Drive Times & Data-Processing Stages \\ \hline
  Garden & Utility Function Reusable Structure Discrete Components \\ \hline
  2-Player Game & Discrete Components Reusable Structure \\ \hline
  Taxes  & Reusable Structure Discrete Components \\ \hline
\end{tabular}
\captionsetup{position=bottom}
\caption{Summary of Problems and Decomposition Features Ordered By Complexity}
\label{table:assignments}
\end{table}

